ICNLoWPAN -- Named-Data Networking for Low Power IoT Networks

Information Centric Networking is considered a promising communication technology for the constrained IoT, but NDN was designed only for standard network infrastructure. In this paper, we design and evaluate an NDN convergence layer for low power lossy links that (1) augments the NDN stateful forwarding with a highly efficient name eliding, (2) devises stateless compression schemes for standard NDN use cases, (3) adapts NDN packets to the small MTU size of IEEE 802.15.4, and (4) generates compatibility with 6LoWPAN so that IPv6 and NDN can coexist on the same LoWPAN links. Our findings indicate that stateful compression can reduce the size of NDN data packets by more than 70% in realistic examples. Our experiments show that for common use cases ICNLoWPAN saves 33% of transmission resources over NDN, and about 20% over 6LoWPAN.

==> figures/styles.tex <==
\tikzset{
    tlfill/.style = { fill=Pastel1-E },
    vfill/.style = { fill=Pastel2-B },
    tlv/.style = { draw, tlfill, font=\sffamily, minimum width=1.75cm, text width=1.75cm, align=center, minimum height=0.60cm, inner sep=0pt, outer sep=0pt },
    stlv/.style = { tlv, font=\sffamily\bfseries, minimum width=0.75cm, text width=0.75cm },
    valbox/.style={ fill=none,
        append after command={
            \pgfextra{
                \begin{scope}
                    \clip (\tikzlastnode.north west) -- ($(\tikzlastnode.north west)!0.4!(\tikzlastnode.north east)$)
                        decorate[decoration={zigzag,segment length=0.5em, amplitude=.5mm}] { -- ($(\tikzlastnode.north west)!0.6!(\tikzlastnode.north east)$) }
                        -- (\tikzlastnode.north east) -- (\tikzlastnode.south east) -- (\tikzlastnode.south west) -- cycle;
                    \fill[#1] ([yshift=.5mm]\tikzlastnode.north west) rectangle ([yshift=.5mm]\tikzlastnode.south east);
                \end{scope}
                \begin{scope}
                    \clip (\tikzlastnode.south west) -- ($(\tikzlastnode.south west)!0.4!(\tikzlastnode.south east)$)
                        decorate[decoration={zigzag,segment length=0.5em, amplitude=.5mm}] { -- ($(\tikzlastnode.south west)!0.6!(\tikzlastnode.south east)$) }
                        -- (\tikzlastnode.south east) -- (\tikzlastnode.north east) -- (\tikzlastnode.north west) -- cycle;
                    \fill[#1] ([yshift=-.5mm]\tikzlastnode.south west) rectangle ([yshift=-.5mm]\tikzlastnode.north east);
                \end{scope}
                \path[draw]
                    (\tikzlastnode.north west) -- ($(\tikzlastnode.north west)!0.4!(\tikzlastnode.north east)$)
                    decorate[decoration={zigzag,segment length=0.5em, amplitude=.5mm}] { -- ($(\tikzlastnode.north west)!0.6!(\tikzlastnode.north east)$) }
                    -- (\tikzlastnode.north east) -- (\tikzlastnode.south east) -- ([xshift=-.01mm]\tikzlastnode.south east);
                \path[draw]
                    (\tikzlastnode.north west) -- (\tikzlastnode.south west) -- ($(\tikzlastnode.south west)!0.4!(\tikzlastnode.south east)$)
                    decorate[decoration={zigzag,segment length=0.5em, amplitude=.5mm}] { -- ($(\tikzlastnode.south west)!0.6!(\tikzlastnode.south east)$) }
                    -- (\tikzlastnode.south east);
            }
        }
    },
    value/.style={ tlv, valbox={vfill}, draw=none, minimum width=3.5cm, text width=3.5cm },
    svalue/.style={ stlv, font=\sffamily, valbox={vfill}, draw=none, minimum width=1.50cm, text width=1.50cm },
    bit/.style = { draw, rectangle, anchor=west, minimum height=0.40cm, minimum width=0.42cm, text width=0.42cm, align=center, font=\sffamily\small, inner sep=0pt, outer sep=0pt },
    mbit/.style = { matrix of nodes, ampersand replacement=\&, nodes={bit}, nodes in empty cells, column sep=-\pgflinewidth,row sep=-\pgflinewidth,anchor=west, inner sep=0pt, outer sep=0pt },
    mbiteven/.style = { mbit,
        column 2/.append style = { nodes = { fill=Pastel1-B } },
        column 3/.append style = { nodes = { fill=Pastel1-B } },
        column 4/.append style = { nodes = { fill=Pastel1-B } },
        column 5/.append style = { nodes = { fill=Pastel1-B } },
        column 6/.append style = { nodes = { fill=Pastel1-C } },
        column 7/.append style = { nodes = { fill=Pastel1-C } },
        column 8/.append style = { nodes = { fill=Pastel1-C } },
        column 9/.append style = { nodes = { fill=Pastel1-C } },
        column 10/.append style = { nodes = { fill=Pastel1-C } },
        column 11/.append style = { nodes = { fill=Pastel1-C } },
        column 12/.append style = { nodes = { fill=Pastel1-C } },
        column 13/.append style = { nodes = { fill=Pastel1-C } },
    },
    mbitodd/.style = { mbit,
        column 2/.append style = { nodes = { fill=Pastel1-A } },
        column 3/.append style = { nodes = { fill=Pastel1-A } },
        column 4/.append style = { nodes = { fill=Pastel1-A } },
        column 5/.append style = { nodes = { fill=Pastel1-A } },
        column 6/.append style = { nodes = { fill=Pastel1-C } },
        column 7/.append style = { nodes = { fill=Pastel1-C } },
        column 8/.append style = { nodes = { fill=Pastel1-C } },
        column 9/.append style = { nodes = { fill=Pastel1-C } },
        column 10/.append style = { nodes = { fill=Pastel1-A } },
        column 11/.append style = { nodes = { fill=Pastel1-A } },
        column 12/.append style = { nodes = { fill=Pastel1-A } },
        column 13/.append style = { nodes = { fill=Pastel1-A } },
    },
    mbitfull/.style = { mbit,
        column 1/.append style = { nodes = { fill=Pastel1-A } },
        column 2/.append style = { nodes = { fill=Pastel1-A } },
        column 3/.append style = { nodes = { fill=Pastel1-A } },
        column 4/.append style = { nodes = { fill=Pastel1-A } },
        column 5/.append style = { nodes = { fill=Pastel1-B } },
        column 6/.append style = { nodes = { fill=Pastel1-B } },
        column 7/.append style = { nodes = { fill=Pastel1-B } },
        column 8/.append style = { nodes = { fill=Pastel1-B } },
        column 9/.append style = { nodes = { fill=Pastel1-A } },
        column 10/.append style = { nodes = { fill=Pastel1-A } },
        column 11/.append style = { nodes = { fill=Pastel1-A } },
        column 12/.append style = { nodes = { fill=Pastel1-A } },
        column 14/.append style = { nodes = { fill=Pastel1-B } },
        column 15/.append style = { nodes = { fill=Pastel1-B } },
        column 16/.append style = { nodes = { fill=Pastel1-B } },
        column 17/.append style = { nodes = { fill=Pastel1-B } },
    },
    traversal/.style = { draw, rectangle, minimum width=2.30cm, minimum height=0.50cm, align=center, text width=2.30cm, font=\scriptsize, inner sep=0pt },
    traversal-154/.style = { traversal, fill=Pastel1-E },
    traversal-6lowpan/.style = { traversal, fill=Pastel2-D, text width=1.125cm, minimum width=1.125cm, font=\tiny },
    traversal-icnlowpan/.style = { traversal, fill=Pastel2-A, text width=1.125cm, minimum width=1.125cm, font=\tiny },
    traversal-ipv6/.style = { traversal, fill=Pastel1-A, text width=1.125cm, minimum width=1.125cm },
    traversal-ndn/.style = { traversal, fill=Pastel1-B, text width=1.125cm, minimum width=1.125cm },
    traversal-app/.style = { traversal, fill=Pastel1-D },
    router/.style = {circle, draw, fill=Pastel1-B, align=center, text centered, inner sep=3pt, node distance=4cm, font=\small},
    smallcell/.style = { draw, align=center, text width=0.900cm, minimum height=4.75mm, inner sep=0pt, anchor=center },
    splitcell/.style = { smallcell, draw=none, fill=none, text width=1.00mm },
    cell/.style = { draw, minimum width=1.60cm, minimum height=5mm, inner sep=0pt, anchor=center },
    smallpit/.style = { matrix of nodes, ampersand replacement=\&, nodes={smallcell}, nodes in empty cells,font=\small,
        row 1/.append style = { nodes = { fill = Pastel1-G, text = black } },
        row 2/.append style = { nodes = { fill = Pastel1-I, text = black } },
    },
}

